ProSpeCT: Provably Secure Speculation for the Constant-Time Policy (Extended version)

We propose ProSpeCT, a generic formal processor model providing provably secure speculation for the constant-time policy. For constant-time programs under a non-speculative semantics, ProSpeCT guarantees that speculative and out-of-order execution cause no microarchitectural leaks. This guarantee is achieved by tracking secrets in the processor pipeline and ensuring that they do not influence the microarchitectural state during speculative execution. Our formalization covers a broad class of speculation mechanisms, generalizing prior work. As a result, our security proof covers all known Spectre attacks, including load value injection (LVI) attacks. In addition to the formal model, we provide a prototype hardware implementation of ProSpeCT on a RISC-V processor and show evidence of its low impact on hardware cost, performance, and required software changes. In particular, the experimental evaluation confirms our expectation that for a compliant constant-time binary, enabling ProSpeCT incurs no performance overhead.

==> more-arrows.tex <==
\usepackage{mathtools}
\usepackage{tikz-cd}
\usetikzlibrary{decorations.pathmorphing}

\makeatletter
\newcommand*{\da@rightarrow}{\mathchar"0\hexnumber@\symAMSa 4B }
\newcommand*{\da@leftarrow}{\mathchar"0\hexnumber@\symAMSa 4C }
\newcommand*{\xdashrightarrow}[2][]{%
  \mathrel{%
    \mathpalette{\da@xarrow{#1}{#2}{}\da@rightarrow{\,}{}}{}%
  }%
}
\newcommand{\xdashleftarrow}[2][]{%
  \mathrel{%
    \mathpalette{\da@xarrow{#1}{#2}\da@leftarrow{}{}{\,}}{}%
  }%
}
\newcommand*{\da@xarrow}[7]{%
  \sbox0{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#1#6\m@th$}%
  \sbox2{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#2#6\m@th$}%
  \sbox4{$#7\dabar@\m@th$}%
  \dimen@=\wd0 %
  \ifdim\wd2 >\dimen@
    \dimen@=\wd2 %
  \fi
  \count@=2 %
  \def\da@bars{\dabar@\dabar@}%
  \@whiledim\count@\wd4<\dimen@\do{%
    \advance\count@\@ne
    \expandafter\def\expandafter\da@bars\expandafter{%
      \da@bars
      \dabar@
    }%
  }%
  \mathrel{#3}%
  \mathrel{%
    \mathop{\da@bars}\limits
    \ifx\\#1\\%
    \else
      _{\copy0}%
    \fi
    \ifx\\#2\\%
    \else
      ^{\copy2}%
    \fi
  }%
  \mathrel{#4}%
}


\newcommand\xrsquigarrow[2]{%
    \mathrel{%
        \begin{tikzpicture}[%
            ,baseline={([yshift=1.5ex]current bounding box.south)}
            ]
        \node [%
            ,inner sep=.44ex
            ,align=center
            ,minimum height=1em
            ] (tmp) {$\scriptstyle #1~$};
        \node [%
            ,inner sep=.44ex
            ,align=center
            ,above=.5em
            ,minimum height=1em
            ] (tmp2) {$\scriptstyle #2~$};
        \path[%
            ,draw,<-
            ,decorate,decoration={%
                ,zigzag
                ,amplitude=0.7pt
                ,segment length=1.2mm,pre length=3.5pt
                }
            ]
        (tmp.north east) -- (tmp.north west);
        \end{tikzpicture}
    }
}

\newcommand\xhookrsquigarrow[2]{%
    \mathrel{%
        \begin{tikzpicture}[%
            ,baseline={([yshift=1.5ex]current bounding box.south)}
            ]
        \node [%
            ,inner sep=.44ex
            ,align=center
            ,minimum height=0em
            ] (tmp) {$\scriptstyle #1~$};
        \node [%
            ,inner sep=.44ex
            ,align=center
            ,above=.5em
            ,minimum height=0em
            ] (tmp2) {$\scriptstyle #2~$};
        \path[%
            ,draw,<-to reversed
            ,decorate,decoration={%
                ,zigzag
                ,amplitude=0.7pt
                ,segment length=1.2mm
                ,pre length=3pt
                ,post length=2pt
                }
            ]
        (tmp.north east) -- (tmp.north west);
        \end{tikzpicture}
    }
}

\newcommand\xlsquigarrow[1]{%
    \mathrel{%
        \begin{tikzpicture}[%
            ,baseline={(current bounding box.south)}
            ]
        \node[%
            ,inner sep=.44ex
            ,align=center
            ] (tmp) {$\scriptstyle #1$};
        \path[%
            ,draw,<-
            ,decorate,decoration={%
                ,zigzag
                ,amplitude=0.7pt
                ,segment length=1.2mm,pre length=3.5pt
                }
            ]
        (tmp.south west) -- (tmp.south east);
        \end{tikzpicture}
        }
      }

\makeatother


==> proof-sketches.tex <==
This section provides proof sketches for \cref{thm:security0} and
\cref{thm:patched_declassification}. Full proofs are available in a technical report.

Notice that the low-projection in \cref{def:sproj} does not differentiate
secrets (\(\slevel{v}{\topsec}\)) from unresolved values (\(\botval\)), i.e.,\
both evaluate to \(\botval\). Therefore, we introduce a new notion of
low-projection for values and register maps \(\rsproj{\cdot}\) and reorder
buffers \(\rsbufproj{\buf}\) that distinguishes these two cases (i.e.,\ such that
for all expression
\(u \in \SVals \cup \{\botval\}.\ \rsproj{u} = \rsproj{u'} \implies (u = \botval \iff u' = \botval)\)).

\bigskip

\noindent{}In particular we have that:
\begin{proposition}\label{prop:defined}
  For two low equivalent buffers \(\rsbufproj{\buf} = \rsbufproj{\buf'}\), two
  low equivalent register maps \(\rsproj{\reg} = \rsproj{\reg'}\), for any
  expression \(e\), \(\semexpr{e}{\aplsan(\buf,\reg)}\) (resp.
  \(\semexpr{e}{\apl(\buf,\reg)}\)) is undefined if and only if
  \(\semexpr{e}{\aplsan(\buf',\reg')}\) (resp.
  \(\semexpr{e}{\apl(\buf',\reg')}\)) is undefined.
\end{proposition}

\securityzero*
\begin{proof}[Proof sketch]
  The proof goes by induction on the number of steps.

  The inductive hypotheses is the following: if the first configuration makes
  \(n-1\) steps, then the second configuration can also make \(n-1\) steps and
  for both configurations we have that:
  \begin{enumerate}
    \item memories are low-equivalent
          (\(\smemproj{\mem_{n-1}} = \smemproj{\mem_{n-1}'}\)),~\label{item:mem}
    \item register maps are low-equivalent
    (\(\rsproj{\reg_{n-1}} = \rsproj{\reg_{n-1}'}\)),~\label{item:reg}
    \item reorder buffers are low-equivalent
    (\(\rsbufproj{\buf_{n-1}} = \rsbufproj{\buf_{n-1}'}\)),~\label{item:buf}
    \item microarchitectural states are equal (\(\micro_{n-1} = \micro_{n-1}'\))~\label{item:micro}.
  \end{enumerate}
  Next, we show that if the first execution can make an additional step, then so
  does the second execution and low equivalence of configurations
  (i.e.,\ \cref{item:mem,item:reg,item:buf,item:micro}) is preserved (which entails
  \cref{thm:security0}).

  Under this inductive hypotheses and assuming \(\update\) is deterministic,
  the \textsc{step} rule selects the same directive in both configurations
  (i.e.,\ \(\nextdir(\micro_{aux})\) where
  \(\micro_{aux} = \update(\micro_{n-1}, \smemproj{\mem_{n-1}}, \sproj{\reg_{n-1}}, \sbufproj{\buf_{n-1}})\)).
  Additionally, for each directive, we show that the rule that is applied is
  determined using only public data. By the inductive hypothesis, all public
  data are equal in both executions so the same rule applies in both executions.
  In particular, for the directive \execute{i}, the low-projection of the
  \(i^{th}\) ROB-instruction is the same in both executions (cf.\
  \cref{item:buf} and \cref{def:sbufproj}) and determines which \textsc{execute}
  rule is applied. %
  Hence the proof proceeds by case analysis on the instruction evaluation rules.

  For each rule, we show that:
  \begin{enumerate*}
    \item if the rule applies in the first configuration then it also applies in
    the second configuration (which, among others, follows from
    \cref{prop:defined}), and
    \item that low-equivalence of configuration (i.e.,\
    \cref{item:mem,item:reg,item:buf,item:micro}) are preserved.
  \end{enumerate*}

  Crucially, we show that predictions (i.e.,\ via \(\predict\)) are only based on
  public values, therefore they are equal in both executions. Moreover,
  microarchitectural states are only updated (via \(\update\)) using public
  values. %
  For instance, for the rule \textsc{execute-load-commit}, it follows from the fact
  that either:
  \begin{itemize}
    \item both configurations are in sequential execution, in which case
          \(\val{a} = \val{a'}\) follows from the hypothesis that the
          program is constant-time;
    \item both configurations are in speculative execution, in which case
          \(\aplsan\) ensures that only public values are forwarded.
    \item other cases are not possible because low-projections of buffers are
          equivalent in both execution (\cref{item:buf}) and speculations are
          disclosed in low-projection of buffers (\cref{def:sbufproj}).
  \end{itemize}




\end{proof}

\thmpatcheddeclassification*
\begin{proof}[Proof sketch]
  The proof is similar to the proof of \cref{thm:security0} except for the rule
  \textsc{retire-store-low}. For this rule, a step in the standard execution
  produces a declassification event \(\declassify{\val{v}}\), corresponding to
  the value stored in low-memory, which is added to the declassification trace.

  In the patched execution, the declassification event is consumed by the rule
  \textsc{retire-store-low-patched}. Crucially, this maintains the invariant
  that low-projections of memories are equal (\cref{item:mem}) and that the
  final declassification trace in the patched execution is empty.
\end{proof}

